An Integrated Development Environment for the Prototype Verification System

The steep learning curve of formal technologies is a well-known barrier to the adoption of formal verification tools in industry. This paper presents VSCode-PVS, a modern integrated development environment for the Prototype Verification System (PVS). This new environment integrates the editing and proof management functionalities of PVS in Visual Studio Code, a popular code editor widely used by software developers. VSCode-PVS provides functionalities that developers expect to find in modern verification tools, but are not available in the standard Emacs front-end of PVS, such as auto-completion, point-and-click navigation of definitions, live diagnostics for errors, and literate programming. The main features and architecture of the environment are presented, along with a comparison with other similar tools.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{R. Monahan, V. Prevosto, J. Proen\c{c}a (Eds.): Formal\\
Integrated Development Environment 2019 (F-IDE 2019)\\
EPTCS 310, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.310.5}{10.4204/EPTCS.310.5}}
\pdfoutput=1

